A survey for variable young stars with small telescopes: V - Analysis of TXOri, V505Ori, and V510Ori, the HST ULLYSES targets in the $\sigma$Ori cluster

Investigations of the formation of young stellar objects (YSOs) and planets require the detailed analysis of individual sources as well as statistical analysis of a larger number of objects. The Hubble UV Legacy Library of Young Stars as Essential Standards (ULLYSES) project provides such a unique opportunity by establishing a UV spectroscopic library of young high- and low-mass stars in the local universe. Here we analyse optical photometry of the three ULLYSES targets (TXOri, V505Ori, V510Ori) and other YSOs in the $\sigma$Ori cluster taken at the time of the HST observations to provide a reference for those spectra. We identify three populations of YSOs along the line of sight to $\sigma$Ori, separated in parallax and proper motion space. The ULLYSES targets show typical YSO behaviour with pronounced variability and mass accretion rates of the order of 10$^{-8}$M$_\odot$/yr. Optical colours do not agree with standard interstellar reddening and suggest a significant contribution of scattered light. They are also amongst the most variable and strongest accretors in the cluster. V505\,Ori shows variability with a seven day period, indicating an inner disk warp at the co-rotation radius. Uncovering the exact nature of the ULLYSES targets will require improved detailed modelling of the HST spectra in the context of the available photometry, including scattered light contributions as well as non-standard reddening.

==> replyreferee.tex <==
We have carefully considered all comments from the referee on our paper and revised the content accordingly. All changes are highlighted in bold face. Please find below detailed replies to the comments.

> Comments to the Author
> This paper does a thorough job of exploring the variability of these targets, and placing them in context of variability in sigma Ori in general.  It is definitely worthy of publication.
>
> My main high-level comment is to make the authors aware that there is another public, high quality photometric dataset that includes these stars: observations from TESS, the Transiting Exoplanet Survey Satellite.  TESS observed the field containing these targets in both Sector 6 (2018-Dec-11 to 2019-Jan-07) and Sector 32 (2020-Nov-19 to 2020-Dec-17).  The latter is significant because it overlaps the HST observations and includes the time period most heavily discussed in the paper.  While TESS does not provide any color information, both the sampling (every 30 minutes in Sector 6 and every 10 minutes in Sector 32, almost continuously for a month) and photometric precision are significantly better than what can be achieved from the ground, and they reveal variability on shorter timescales than the ground-based data are able to.
>
> I realize that revising the paper to take the TESS data into account would be a significant undertaking, and I leave it to the authors to decide whether or not they want to do that.  But at the very least they should be aware of its existence and acknowledge it in the paper.  If they choose not to address those data in this paper, they may still want to test some of their statements in the paper against what is shown by the TESS lightcurves to make sure they still hold up.  For example, the statement on page 8 (Sec. 5.3 on V505 Ori) that "the maxima are rounded" is clearly contradicted by the TESS data, which show sharp maxima in most peaks in both sectors.
>
> Since I extracted the TESS light curves from the full-frame images to satisfy my own curiosity, I have taken the liberty of including them along with this report to help the authors judge for themselves what they would like to do about the TESS data.  These were extracted from the TESS full-frame images using the lightkurve python package, using simple background subtraction from creating a background mask from sky pixels near the target.  (These are bright stars by TESS standards, so the background subtraction did not fundamentally change the appearance of the light curves, other than eliminating a spike near the data gap at the middle of each sector's timespan.)

Reply: We very much appreciate the comments regarding the TESS data as well as the light curves attached to the report. The HST data has been coordinated with the TESS data, and another group from the ULLYSES collaboration is already working on a separate publication investigating the TESS light curves. We thus will not include any of this analysis in our paper, but note it in Sect.3 and also revise the text in other places when sub-day variability is discussed.


> A few general comments about the figures, which apply throughout the paper:
> 
> - There are many figures that include separate panels for the three targets TX Ori, V505 Ori, and V510 Ori. The identifications of which panel is for which target are always given in the figure captions, but it would be helpful to the reader to include that information on the figures themselves.

Reply: We had already experimented with labelling each figure with the source name. There are several problems with this. In almost all cases it is impossible to place a label in the same corner of the plot without covering up some of the data points. Having the labels in different corners looks very untidy. And creating the space in the panels for the labels squashes the data into a much smaller area. We thus decided against the labels. Note that for these reasons we have kept the same order of the sources in all figures/tables and consistently also used the same order when discussing the objects in the text to avoid any confusion.

> - There are a number of figures where the choice of colors makes it hard to read the figure.  In Figure 1, for example, it is very difficult for me to distinguish the dark blue from the dark green points, since both are quite dark.  The dark colors used in Figure 9 are similarly hard to read.  I have normal color vision, and I still struggled with some figures, but readers with red-green color blindness (about 7-10% of the population) would have a hard time with the colormaps used in many of the figures.  I encourage the authors to consider alternate colormaps for their figures, to make them more accessible to a wider range of readers.

Reply: We agree that in some cases colours are hard to distinguish in the plots. It turns out that some of this gets much worse/better depending on the screen used to view the plots. We nevertheless have checked all Figures and find that with one exception there is additional information such as symbol shape and symbol values (at times listed in an accompanying table) that will allow to distinguish the colours. We agree that in Fig.1. this can be difficult. We have hence redone all the panels in this figure using light-green instead of green symbols to address the issues in the referee's comments. The description in the figure caption and text has been adapted accordingly.

> The authors took data in the Sloan u filter, but for reasons that aren't stated they choose to refer to this data throughout the paper as U, which unfortunately is the name of a different filter. While they say in passing in the text that this is what they are doing, I think this choice will only promote confusion among readers of this paper in the future.  When I look at a figure or table in a paper and it says (for example) "B-V", I generally take that at face value and don't feel the need to scour the paper in detail to determine if those were the filters used, or if that really means B - g' and that the authors have simply chosen to call the latter filter "V".  I recommend that the data (in all bands) be referred to by the filter name, following the usual astronomical convention.  I note that the authors also use the Johnson U filter characteristics when converting their Sloan u magnitudes to fluxes in Section 5.6, which is confusing; the two filters have similar bandpasses, but zero points that differ by 0.85 mags (e.g. Chonis & Gaskell 2008).  If there is something about how the u data were taken (perhaps the standards used?) that means that they should more properly be considered as Johnson U magnitudes, then that needs to be explained in more detail in the paper.

Reply: We agree with the referee that there is some confusion, which has been caused by a lack of details in our description in Sect.3. For each field and filter we have a reference frame against which all other images in the same/similar filter are calibrated against. The magnitudes in the reference frame are then shifted into the Johnson UBV and Cousins RI system, hence the use of UBVRI for the filters. Colour terms are determined for each image using the method described in Evitts et al. (2020). We have revised the description of this in the text of Sect.3. Note that with one exception, all our analysis only relies on magnitude changes, and is thus not sensitive to zero-point off-sets. Only the mass accretion rate determination requires the correct zero points. Errors in those will change the absolute values for Macc, but keep the relative values. 

> Detailed comments:

> Section 2.2:  This text presents a significant amount of data (magnitudes in different filters, spectral types, references) that might be more efficiently presented in tabular form.

Reply: We agree with this statement in that there is a large amount of information in this section. We have tried initially to collate the values and references in a table. However, no matter how such a table is organised, it seems to take up more space than the text in the section, i.e. half a page. We have hence left the Section as is was.

> Page 3, footnote: give the URL in the footnote (rather than just hyperlinking the displayed text)

Reply: changed as requested

> Page 3, Section 3: see my comment above about u vs. U.

Reply: Changed according to our comments to the main point about this.

> Page 3, column 1, last paragraph:  "The vast majority of images for this field [have] been taken ... and hence [have]... "

Reply: Yes, changed as suggested.

> Second column, first sentence:  tree -> three

Reply: changed

> P. 4, first column, middle: "much sparser populated" -> "much more sparsely populated"

Reply: changed

> last full paragraph:  "Thus, indicating a difference in velocity distributions."  Not a full sentence, revise.

Reply: We have re-worded that 'sentence'.

> P. 8, first paragraph: "This is indicating large dust grains or unusual scattering properties."   Just a few sentences prior to this, the authors have concluded that the extinction models do not explain what they see in those sources.  Therefore, the interpretation of the data in the context of those same models doesn't make sense here.

Reply: This is correct. We have removed the sentence.

> Next paragraph:  "The turning in colour behaviour is usually interpreted as a sign that increased extinction..."  Please cite references for this interpretation.

Reply: Yes, we added a reference.

> P. 8, Sec. 5.3:  The very small error bar on the period (only 10 minutes on a 7-day period) is surprising.  Given the scatter and broad peaks of the data shown in Figure 5, and the sampling of the data, it's hard to believe that the period is known this precisely, especially if only one season of data is being used here.  Please clarify how the period uncertainty was determined.

Reply: Correct we did not state that. The error is the RMS scatter from the 4 periods determined for each of the filters, which are independent datasets. We have added a note in the text.

> Sec. 5.3, second paragraph:  As noted above, some of the peaks in the TESS light curves are very sharp, so consider revising here even if the TESS data are not used.

Reply: Yes we have done that as part of the changes regarding the TESS data. We have reworded the text slightly and added some additional notes.

> Sec. 5.5, pp. 11-12:  "This means, the range of variability of the source is entirely governed by the periodic nature of the object."  It's not clear to me what this sentence means.  Are the authors saying that the periodic variability has larger amplitude than variability at other timescales?

Reply: We have reworded the sentence to make it more clear. 

> Next paragraph: "increases steady" -> increases steadily

Reply: changed as requested

> p. 14, bottom of first column: "about one quarter of YSOs [are] more variable"

Reply: changed as requested

> Next column: "to a large extend" -> extent

Reply: changed as requested
